Out-of-Candidate Rectification for Weakly Supervised Semantic Segmentation

Weakly supervised semantic segmentation is typically inspired by class activation maps, which serve as pseudo masks with class-discriminative regions highlighted. Although tremendous efforts have been made to recall precise and complete locations for each class, existing methods still commonly suffer from the unsolicited Out-of-Candidate (OC) error predictions that not belongs to the label candidates, which could be avoidable since the contradiction with image-level class tags is easy to be detected. In this paper, we develop a group ranking-based Out-of-Candidate Rectification (OCR) mechanism in a plug-and-play fashion. Firstly, we adaptively split the semantic categories into In-Candidate (IC) and OC groups for each OC pixel according to their prior annotation correlation and posterior prediction correlation. Then, we derive a differentiable rectification loss to force OC pixels to shift to the IC group. Incorporating our OCR with seminal baselines (e.g., AffinityNet, SEAM, MCTformer), we can achieve remarkable performance gains on both Pascal VOC (+3.2%, +3.3%, +0.8% mIoU) and MS COCO (+1.0%, +1.3%, +0.5% mIoU) datasets with negligible extra training overhead, which justifies the effectiveness and generality of our OCR.

==> codes/tmp.tex <==
\begin{algorithm}[t]
\caption{Out-of-Candidate Rectification (OCR): PyTorch-like Pseudocode}
\label{alg:code}
\algcomment{
\textbf{Notes}: \texttt{mm} is matrix multiplication. \texttt{k.t()} is \texttt{k}'s transpose. The prediction head is excluded from \texttt{f\_k} (and thus the momentum update).
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
\begin{lstlisting}[language=python]
# im_gt: image-level tag labels (C x H x W)
# pred: network output logit ((C + 1) x H x W)
# M: prior correlation matrix ((C + 1) x (C + 1))
# tau: IC group useless classes filter threshold
# delta: the margin value

def get_ic_ids(im_gt):
    return torch.cat([0, torch.nonzero(im_gt) + 1])

def get_oc_ids(im_gt):
    return torch.nonzero(1 - im_gt) + 1

# single pixel behavior
def ic_gp_build(pix_logit, ic_class_ids):
    pix_prob = torch.softmax(pix_logit)
    ic_gp_prob = pix_prob[ic_class_ids]
    ic_filter_mask = torch.zeros(len(ic_class_ids))
    # 1. Anchor Predictions and Classes
    anchor_prob, anchor_id = torch.max(ic_gp_prob)
    ic_filter_mask[anchor_id] = 1
    # 2. utilize correlation for filtering
    cond = (anchor_prob - pix_prob * M[anchor_id]) < tau
    ic_filter_mask[cond] = 1
    
    return ic_filter_mask

# Out-of-Candidate Rectification Loss
def ocr_loss(pred, im_gt):
    # OC pixels selection mask
    clean_pred = pred.detach().clone()
    clean_pred[1:] = clean_pred[1:] * im_gt # ignore background class
    oc_mask = clean_pred != pred
    
    # Adaptive Group Split
    ic_gp_logits, ic_filter_mask = ic_gp_build(pred, im_gt) # 
    oc_gp_logits = oc_gp_build(pred, im_gt)
    
    # Rectification Loss
    l_rec = torch.log(1 + 
    
    spatial_ic_filter_mask = torch.zeros((len(ic_class_ids), H, W))
    for i in range(H):
        for j in range(W):
            spatial_ic_filter_mask[:, i, j] = ic_gp_build(pred, ic_class_ids)
    
    ic_gp_logits = pred[ic_class_ids] * spatial_ic_filter_mask
    ## OC group build
    oc_class_ids = get_oc_ids(im_gt)
    oc_gp_logits = pred[oc_class_ids]

    # Loss Calculation

\end{lstlisting}
\end{algorithm}

==> tab/abl_margin_alpha.tex <==
\begin{table}[t]
\caption{The performance (mIoU (\%)) influence of the margin value $ \Delta $ and the loss coefficient $ \alpha $ for penalizing loss $ L_{penalize} $. This study is based on SEAM and the results are evaluated on Pascal VOC \textit{val} split.}
\label{tab:abl_margin_alpha}
\small
\centering
\begin{tabular}{lcccccc}
\toprule 
$ \downarrow \alpha $ / $ \Delta \rightarrow $   & 0 & 0.5 & 2.0 & 4.0 & 6.0 & 8.0 \\
\midrule
0.1           & 64.9 & 65.5 & 66.0 & 66.2 & 66.1 & 64.5 \\
1             & 67.1 & 67.6 & 67.8 & 63.9 & 62.1 & 61.3 \\
10            & 66.3 & 65.2 & 65.7 & 60.3 & 56.5 & 49.4 \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}
